Near-Online Multi-target Tracking with Aggregated Local Flow Descriptor

In this paper, we focus on the two key aspects of multiple target tracking problem: 1) designing an accurate affinity measure to associate detections and 2) implementing an efficient and accurate (near) online multiple target tracking algorithm. As the first contribution, we introduce a novel Aggregated Local Flow Descriptor (ALFD) that encodes the relative motion pattern between a pair of temporally distant detections using long term interest point trajectories (IPTs). Leveraging on the IPTs, the ALFD provides a robust affinity measure for estimating the likelihood of matching detections regardless of the application scenarios. As another contribution, we present a Near-Online Multi-target Tracking (NOMT) algorithm. The tracking problem is formulated as a data-association between targets and detections in a temporal window, that is performed repeatedly at every frame. While being efficient, NOMT achieves robustness via integrating multiple cues including ALFD metric, target dynamics, appearance similarity, and long term trajectory regularization into the model. Our ablative analysis verifies the superiority of the ALFD metric over the other conventional affinity metrics. We run a comprehensive experimental evaluation on two challenging tracking datasets, KITTI and MOT datasets. The NOMT method combined with ALFD metric achieves the best accuracy in both datasets with significant margins (about 10% higher MOTA) over the state-of-the-arts.

==> fig_examples.tex <==
\begin{tabular}{c@{\hspace{1mm}}c@{\hspace{1mm}}c}
\includegraphics[width=0.32\linewidth, trim =18mm 118mm 18mm 107mm, clip]{figures/examples/0001-00000224.pdf} &
\includegraphics[width=0.32\linewidth, trim =18mm 118mm 18mm 107mm, clip]{figures/examples/0004-00000028.pdf} &
\includegraphics[width=0.32\linewidth, trim =18mm 118mm 18mm 107mm, clip]{figures/examples/p0013-00000258.pdf} \\
\includegraphics[width=0.32\linewidth, trim =18mm 118mm 18mm 107mm, clip]{figures/examples/0002-00000116.pdf} &
\includegraphics[width=0.32\linewidth, trim =18mm 118mm 18mm 107mm, clip]{figures/examples/b0016-00000171.pdf} &
\includegraphics[width=0.32\linewidth, trim =18mm 118mm 18mm 107mm, clip]{figures/examples/p0017-00000048.pdf} \\
\includegraphics[width=0.32\linewidth, trim =18mm 118mm 18mm 107mm, clip]{figures/examples/0020-00000109.pdf} &
\includegraphics[width=0.32\linewidth, trim =18mm 118mm 18mm 107mm, clip]{figures/examples/b0015-00000054.pdf} &
\includegraphics[width=0.32\linewidth, trim =18mm 118mm 18mm 107mm, clip]{figures/examples/p0019-00000233.pdf} \\
\includegraphics[width=0.32\linewidth, trim =18mm 16mm 60mm 135mm, clip]{figures/examples/error1.pdf} & 
\includegraphics[width=0.32\linewidth, trim =18mm 16mm 60mm 135mm, clip]{figures/examples/error2.pdf} & 
\includegraphics[width=0.32\linewidth, trim =18mm 16mm 60mm 135mm, clip]{figures/examples/error3.pdf} 
\end{tabular}
\caption{Qualitative tracking results of {\bf NOMT} on the KITTI dataset. The first three rows shows typical successful tracking results and the last row shows failure cases. 
Current frame location is shown as a bounding box and the bottom points of previous 10 frames are shown as dotted trajectories. The result demonstrates the robustness of our algorithm under various challenges, e.g. rapid camera motion, target occlusion, cluttered scene, etc.
The method fails in very challenging cases, when a target do not follow linear motion while occluded, adjacent two targets have very similar appearance, or the time and location of a target appears are identical to those of the other disappears.
Color shows target identity. The figure is best shown in color. We provide more result videos in the supplemental materials.}
\vspace{-3mm}
\label{fig:qualitative}

==> tab_feat.tex <==
\begin{center}
{\scriptsize
\begin{tabular}{|c||c|ccc||c|ccc||c|ccc|}
\hline
Object & \multicolumn{4}{c||}{Car} & \multicolumn{4}{c||}{Pedestrian} & \multicolumn{4}{c|}{Cyclist} \\
\hline
Mode & Full & $\minus$ALFD & $\minus$TD & $\minus$AS & Full & $\minus$ALFD & $\minus$TD & $\minus$AS & Full & $\minus$ALFD & $\minus$TD & $\minus$AS \\
\hline
\hline
F1 $\uparrow$ & 76.9 \% & {\bf 74.0} \% & 76.3 \% & 76.2 \% 
& 73.8 \% & {\bf 71.2} \% & 73.3 \% & 73.2 \%
& 73.5 \% & {\bf 70.8} \% & 72.9 \% & 72.8 \% \\
\hline
\hline
MOTA $\uparrow$ & 61.2 \% & {\bf 57.5} \% & 60.4 \% & 60.3 \% 
& 55.1 \% & {\bf 51.6} \% & 54.3 \% & 54.1 \% 
& 54.7 \% & {\bf 51.3} \% & 53.9 \% & 53.8 \% 
\\
MOTP $\uparrow$ & {\bf 79.7} \% & 80.0 \% & 79.8 \% & 79.8 \% 
& {\bf 77.8} \% & 78.0 \% & {\bf 77.8} \% & 77.9 \% 
& {\bf 77.9} \% & 78.1 \% & {\bf 77.9} \% & 78.0 \% \\
MT $\uparrow$ & 31.1 \% & {\bf 21.6} \% & 29.5 \% & 28.6 \% 
& 26.5 \% & {\bf 16.3} \% & 24.1 \% & 25.3 \% 
& 27.7 \% & {\bf 24.8} \% & 25.0 \% & 25.0 \% \\
ML $\downarrow$ & 25.2 \% & {\bf 30.0} \% & 24.9 \% & 24.8 \% 
& 27.7 \% & {\bf 31.9} \% & 25.9 \% & 25.9 \% 
& {\bf 41.3} \% & 38.7 \% & 38.5 \% & 41.2 \% \\
IDS $\downarrow$ & 15 & {\bf 110} & 28 & 44 
& 49 & {\bf 215} & 58 & 113 
& 49 & {\bf 220} & 63 & 114 \\
FRAG $\downarrow$ & 106 & {\bf 240} & 130 & 168 
& 427 & {\bf 624} & 430 & 550 
& 430 & {\bf 634} & 439 & 555 \\ 
\hline
\end{tabular}
}
\caption{Experimental analysis on the contribution of each potential component. 
We remove one match potential in each experiment.
The worst numbers are bold-faced to highlight the contribution of the potential.
We use $\tau = 10$ in these experiments.} 
\label{tab:feat}
\vspace{-4mm}
\end{center}

==> tab_tau.tex <==
\begin{center}
{\scriptsize
\begin{tabular}{|c||c|cccccccccc|}
\hline
$\tau$ (frames) & HM & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\
\hline
\hline
% Rec. $\uparrow$ & 61.1 \% & 62.2 \% & 62.1 \% & 62.4 \% & 63.0 \% & 63.5 \% & 63.5 \% & 63.6 \% & 63.6 \% & {\bf 63.7} \% & 63.6 \% \\
% Prec. $\uparrow$ & 96.07 \% & 96.5 \% & {\bf 97.7} \% & 97.2 \% & 97.5 \% & 97.2 \% & 97.3 \% & 97.1 \% & 96.8 \% & 97.2 \% & 97.1 \% \\
F1 $\uparrow$ & 74.8 \% & 75.6 \% & 75.9 \% & 76.0 \% & 76.6 \% & 76.8 \% & 76.9 \% & 76.9 \% & 76.8 \% & {\bf 77.0} \% & 76.9 \% \\
\hline
\hline
MOTA $\uparrow$ & 57.8 \% & 59.6 \% & 60.4 \% & 60.3 \% & 61.1 \% & 61.2 \% & 61.2 \% & 61.2 \% & 61.0 \% & {\bf 61.4} \% & 61.2 \%\\
MOTP $\uparrow$ & 79.6 \% & {\bf 79.9} \% & 79.9 \% & 79.9 \%	 & 79.8 \% & 79.7 \% & 79.7 \% & 79.7 \% & 79.7 \% & 79.7 \% & 79.7 \% \\
MT $\uparrow$ & 26.8 \%  &  28.7 \% & 29.3 \% & 29.7 \% & 30.2 \% & 30.8 \% & 30.8 \% & 30.8 \% & 30.8 \% & 30.8 \% & {\bf 31.1} \% \\
ML $\downarrow$ & 28.1 \% & 25.9 \% & 26.2 \% & 26.2 \% & 25.4 \% & {\bf 25.2} \% & 25.4 \% & 25.6 \% & {\bf 25.2} \% & 25.6 \% & {\bf 25.2} \% \\
IDS $\downarrow$ & 32 & 222 & 175 & 171 & 27 &	17 & 15 & {\bf 14} & {\bf 14} & {\bf 14} & 15 \\
FRAG $\downarrow$ & 153 & 332 & 271	& 266	& 123	& 115	& 109	& 109	& 106	& {\bf 102}	& 106 \\
\hline
\hline
Comp. $\downarrow$ & {\bf 0.089} & 0.104 & 0.138 & 0.178 & 0.211 & 0.237 & 0.215 & 0.232 & 0.272 & 0.299 & 0.277 \\
Latency $\downarrow$ & {\bf 0.16} & 0.32 & 0.43 & 0.66 & 0.88 & 1.18 & 1.51 & 1.86 & 2.21 & 2.61 & 3.03 \\
% Latency	& 0.32 +- 1.05 & 0.43 / 1.03	 & 0.66 / 1.30 & 0.88 / 1.58 & 1.18 / 1.95 & 1.51 / 2.31 & 1.86 / 2.67 & 2.21 / 3.04 & 2.61 / 3.43 & 3/03 / 3.84 \\ 
\hline
\end{tabular}
}
\caption{Tracking accuracy over $\tau$ on the KITTI Car tracking training set. The best numbers in each row are bold-faced.} \label{tab:tau}
\vspace{-6mm}
\end{center}
